The Rotation of M Dwarfs Observed by the Apache Point Galactic Evolution Experiment

We present the results of a spectroscopic analysis of rotational velocities in 714 M dwarf stars observed by the SDSS III Apache Point Galactic Evolution Experiment (APOGEE) survey. We use a template fitting technique to estimate $v\sin{i}$ while simultaneously estimating $\log{g}$, $[\text{M}/\text{H}]$, and $T_{\text{eff}}$. We conservatively estimate that our detection limit is 8 km s$^{-1}$. We compare our results to M dwarf rotation studies in the literature based on both spectroscopic and photometric measurements. Like other authors, we find an increase in the fraction of rapid rotators with decreasing stellar temperature, exemplified by a sharp increase in rotation near the M$4$ transition to fully convective stellar interiors, which is consistent with the hypothesis that fully convective stars are unable to shed angular momentum as efficiently as those with radiative cores. We compare a sample of targets observed both by APOGEE and the MEarth transiting planet survey and find no cases were the measured $v\sin{i}$ and rotation period are physically inconsistent, requiring $\sin{i}>1$. We compare our spectroscopic results to the fraction of rotators inferred from photometric surveys and find that while the results are broadly consistent, the photometric surveys exhibit a smaller fraction of rotators beyond the M$4$ transition by a factor of $\sim 2$. We discuss possible reasons for this discrepancy. Given our detection limit, our results are consistent with a bi-modal distribution in rotation that is seen in photometric surveys.

==> table_myvsini_final_full.tex <==
\tablecaption{\vsinie Results\label{table:myvsini}}
\tablenum{4}
\tablehead{\colhead{2MASS ID} &
\colhead{RA} &
\colhead{DEC} &
\colhead{\taspcap} &
\colhead{T$_{\textrm{eff, VFIT}}$} &
\colhead{$\met_{\textrm{VFIT}}$} &
\colhead{$\logg_{\textrm{VFIT}}$} &
\colhead{$\vsini_{\textrm{VFIT}}$} \\
\colhead{} & 
\colhead{(degrees J2000)} &
\colhead{(degrees J2000)} &
\colhead{(K)} &
\colhead{(K)} &
\colhead{(dex)} &
\colhead{(dex)} &
\colhead{(\kms)}} 
\startdata
J00004701$+$1624101 & $0.19587600$ & $16.402811$ & $3725$ & $3800$ & $+0.5$ & $5.0$ & $<8.0$\\
J00012694$+$1639052 & $0.36228900$ & $16.651464$ & $3677$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J00034394$+$8606422 & $0.93308800$ & $86.111732$ & $2893$ & $2800$ & $-0.0$ & $5.0$ & $13.2\pm1.5$\\
J00070982$+$0007402 & $1.7909290$ & $0.12785100$ & $3656$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J00121468$+$7138322 & $3.0611740$ & $71.642281$ & $3296$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J00131578$+$6919372 & $3.3157730$ & $69.327003$ & $3365$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J00182072$+$6730342 & $4.5863700$ & $67.509514$ & $3321$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J00185999$+$5836527 & $4.7499940$ & $58.614662$ & $3227$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J00211310$+$7418403 & $5.3046070$ & $74.311218$ & $3414$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J00220064$+$6154200 & $5.5026750$ & $61.905575$ & $3361$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J00222083$+$8619567 & $5.5868170$ & $86.332428$ & $3154$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J00241572$+$6549199 & $6.0655410$ & $65.822220$ & $3691$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J00243855$+$5119224 & $6.1606360$ & $51.322895$ & $3504$ & $3500$ & $-0.0$ & $5.0$ & $<8.0$\\
J00251480$+$6225017 & $6.3116950$ & $62.417149$ & $3092$ & $3100$ & $-0.5$ & $5.0$ & $<8.0$\\
J00251602$+$5422547 & $6.3167660$ & $54.381882$ & $2610$ & $2600$ & $-0.0$ & $5.0$ & $<8.0$\\
J00252974$+$5412240 & $6.3739560$ & $54.206673$ & $3342$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J00255540$+$5749320 & $6.4808560$ & $57.825562$ & $3400$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J00255888$+$5559296 & $6.4953360$ & $55.991581$ & $3589$ & $3500$ & $-0.0$ & $4.5$ & $11.5\pm1.5$\\
J00262872$+$6747026 & $6.6196670$ & $67.784073$ & $3756$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J00270673$+$4941531 & $6.7780790$ & $49.698093$ & $3297$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J00285391$+$5022330 & $7.2246660$ & $50.375839$ & $3236$ & $3200$ & $+0.5$ & $5.0$ & $14.2\pm1.5$\\
J00301250$+$5028392 & $7.5520980$ & $50.477570$ & $3209$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J00303669$+$7020584 & $7.6528900$ & $70.349564$ & $3465$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J00312793$+$6139333 & $7.8664010$ & $61.659252$ & $2743$ & $2600$ & $-0.0$ & $5.0$ & $<8.0$\\
J00313293$+$6152504 & $7.8872350$ & $61.880680$ & $3383$ & $3400$ & $-0.5$ & $4.5$ & $<8.0$\\
J00321574$+$5429027 & $8.0655900$ & $54.484100$ & $3249$ & $3200$ & $+0.5$ & $5.0$ & $<8.0$\\
J00322612$+$5019121 & $8.1088380$ & $50.320049$ & $3305$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J00330661$+$5753452 & $8.2775770$ & $57.895893$ & $3395$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J00331747$+$6327504 & $8.3228160$ & $63.464008$ & $3137$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J00333033$+$7054422 & $8.3764000$ & $70.911728$ & $3383$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J00333911$+$5116451 & $8.4129680$ & $51.279198$ & $3658$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J00334085$+$6241566 & $8.4202180$ & $62.699066$ & $3858$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J00340186$+$5040537 & $8.5077700$ & $50.681602$ & $3383$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J00350487$+$5953079 & $8.7703200$ & $59.885548$ & $3225$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J00372598$+$5133072 & $9.3582810$ & $51.552025$ & $3862$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J00380386$+$1656028 & $9.5160860$ & $16.934135$ & $3396$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J00383388$+$5127579 & $9.6411840$ & $51.466103$ & $3423$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J00391896$+$5508132 & $9.8290380$ & $55.137009$ & $3145$ & $3200$ & $-0.5$ & $4.5$ & $<8.0$\\
J00444820$+$1830403 & $11.200835$ & $18.511221$ & $3636$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J01094190$+$8612302 & $17.424610$ & $86.208412$ & $3263$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J01195227$+$8409327 & $19.967825$ & $84.159111$ & $3046$ & $3000$ & $-0.0$ & $5.0$ & $<8.0$\\
J01232542$+$1638384 & $20.855939$ & $16.644014$ & $3265$ & $3300$ & $-0.0$ & $5.0$ & $16.8\pm1.5$\\
J01251185$+$1711483 & $21.299404$ & $17.196775$ & $3771$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J01285381$+$1803284 & $22.224244$ & $18.057915$ & $3641$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J01311367$+$1654026 & $22.806999$ & $16.900745$ & $3506$ & $3500$ & $+0.5$ & $5.5$ & $<8.0$\\
J01382032$+$6246328 & $24.584698$ & $62.775799$ & $3297$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J02040123$+$4855372 & $31.005161$ & $48.927025$ & $3319$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J02041225$+$1424094 & $31.051062$ & $14.402626$ & $3803$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J02043199$+$1442210 & $31.133313$ & $14.705858$ & $3633$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J02073745$+$1354497 & $31.906080$ & $13.913806$ & $3774$ & $3900$ & $+0.5$ & $5.0$ & $<8.0$\\
J02081218$+$1508424 & $32.050754$ & $15.145118$ & $3174$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J02081366$+$4949023 & $32.056958$ & $49.817318$ & $2824$ & $2600$ & $-0.0$ & $5.0$ & $<8.0$\\
J02085359$+$4926565 & $32.223315$ & $49.449055$ & $3340$ & $3300$ & $+0.5$ & $5.0$ & $22.9\pm1.5$\\
J02090912$+$1435362 & $32.288026$ & $14.593390$ & $3608$ & $3700$ & $-0.0$ & $5.0$ & $<8.0$\\
J02122001$+$1249287 & $33.083411$ & $12.824662$ & $3459$ & $3700$ & $+0.5$ & $5.5$ & $<8.0$\\
J02144781$+$5334438 & $33.699241$ & $53.578857$ & $3333$ & $3400$ & $-0.5$ & $5.0$ & $<8.0$\\
J02170514$+$5434535 & $34.271423$ & $54.581551$ & $3116$ & $3100$ & $-1.0$ & $5.0$ & $<8.0$\\
J02210709$+$5457023 & $35.279558$ & $54.950665$ & $3401$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J02250239$+$6006593 & $36.259971$ & $60.116489$ & $3385$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J02362715$+$5528349 & $39.113162$ & $55.476364$ & $3382$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J02410716$+$5423087 & $40.279860$ & $54.385777$ & $3773$ & $3900$ & $+0.5$ & $5.0$ & $<8.0$\\
J02412178$+$5437381 & $40.340787$ & $54.627274$ & $3272$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J02420546$+$5506554 & $40.522786$ & $55.115398$ & $3441$ & $3500$ & $-0.0$ & $5.0$ & $<8.0$\\
J02465257$+$5619505 & $41.719054$ & $56.330704$ & $3378$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J03023866$+$6228135 & $45.661089$ & $62.470444$ & $3398$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J03044335$+$6144097 & $46.180640$ & $61.736034$ & $3420$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J03062774$+$6254388 & $46.615589$ & $62.910782$ & $3165$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J03100122$+$6306218 & $47.505084$ & $63.106079$ & $3290$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J03140624$+$5728568 & $48.526026$ & $57.482445$ & $3412$ & $3400$ & $+0.5$ & $5.5$ & $<8.0$\\
J03143718$+$0030111 & $48.654951$ & $0.50308600$ & $3563$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J03150093$+$0103083 & $48.753909$ & $1.0523240$ & $3621$ & $3600$ & $-1.0$ & $4.5$ & $<8.0$\\
J03150691$+$4016231 & $48.778809$ & $40.273090$ & $3407$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J03152943$+$5751330 & $48.872662$ & $57.859180$ & $3312$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J03184739$+$0803206 & $49.697497$ & $8.0557450$ & $3728$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J03190500$+$6149280 & $49.770839$ & $61.824467$ & $3355$ & $3300$ & $-0.0$ & $5.0$ & $8.55\pm1.5$\\
J03192308$+$0215421 & $49.846174$ & $2.2617200$ & $3768$ & $3800$ & $-0.0$ & $4.5$ & $14.1\pm1.5$\\
J03192872$+$6156045 & $49.869708$ & $61.934605$ & $3237$ & $3200$ & $+0.5$ & $5.5$ & $17.1\pm1.5$\\
J03204249$+$0902099 & $50.177068$ & $9.0360940$ & $3338$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J03212176$+$7958022 & $50.340691$ & $79.967285$ & $3586$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J03223455$+$5049115 & $50.643964$ & $50.819885$ & $3319$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J03234657$+$0805058 & $50.944073$ & $8.0849690$ & $2895$ & $3000$ & $-0.5$ & $5.5$ & $<8.0$\\
J03254578$+$0951591 & $51.440775$ & $9.8664380$ & $3431$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J03264491$+$7108292 & $51.687157$ & $71.141464$ & $3328$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J03280163$+$5226180 & $52.006827$ & $52.438358$ & $3780$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J03282794$+$0813110 & $52.116440$ & $8.2197380$ & $3135$ & $3100$ & $+0.5$ & $5.5$ & $<8.0$\\
J03300766$+$4711159 & $52.531921$ & $47.187763$ & $3041$ & $3000$ & $-0.0$ & $5.0$ & $8.39\pm1.5$\\
J03305473$+$7041145 & $52.728069$ & $70.687378$ & $3270$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J03355099$+$7140275 & $53.962466$ & $71.674332$ & $3192$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J03380791$+$4727134 & $54.532968$ & $47.453743$ & $3295$ & $3300$ & $-0.5$ & $4.5$ & $<8.0$\\
J03391302$+$4635276 & $54.804269$ & $46.591000$ & $3402$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J03391968$+$3251001 & $54.832001$ & $32.850037$ & $3500$ & $3500$ & $+0.5$ & $5.5$ & $<8.0$\\
J03400164$+$4638456 & $55.006837$ & $46.646011$ & $3637$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J03414157$+$3130583 & $55.423244$ & $31.516216$ & $3370$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J03424828$+$3040342 & $55.701172$ & $30.676168$ & $3040$ & $3000$ & $-0.0$ & $5.0$ & $8.86\pm1.6$\\
J03425617$+$2515528 & $55.734068$ & $25.264671$ & $3168$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J03441913$+$7126195 & $56.079740$ & $71.438751$ & $3582$ & $3600$ & $+0.5$ & $5.0$ & $<8.0$\\
J03463676$+$3110459 & $56.653194$ & $31.179443$ & $3577$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J03481149$+$3054134 & $57.047896$ & $30.903734$ & $3311$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J03553536$+$5002402 & $58.897358$ & $50.044521$ & $3326$ & $3400$ & $-0.5$ & $4.5$ & $<8.0$\\
J03553688$+$5214291 & $58.903693$ & $52.241417$ & $3403$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J03583626$+$5201252 & $59.651122$ & $52.023670$ & $3693$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J04010755$+$5123196 & $60.281459$ & $51.388779$ & $3324$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J04030024$+$5238026 & $60.751031$ & $52.634060$ & $3073$ & $3200$ & $-0.5$ & $5.5$ & $<8.0$\\
J04042573$+$5322083 & $61.107229$ & $53.368984$ & $3811$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J04063732$+$7916012 & $61.655503$ & $79.267006$ & $2956$ & $2900$ & $-0.0$ & $5.0$ & $<8.0$\\
J04104186$+$5124238 & $62.674441$ & $51.406612$ & $3349$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J04125880$+$5236421 & $63.245023$ & $52.611698$ & $3206$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J04153706$+$5422491 & $63.904435$ & $54.380318$ & $3957$ & $4000$ & $-0.5$ & $4.5$ & $<8.0$\\
J04204796$+$5624202 & $65.199861$ & $56.405624$ & $2761$ & $2800$ & $-0.0$ & $5.0$ & $<8.0$\\
J04205054$+$4405369 & $65.210593$ & $44.093590$ & $3439$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J04220630$+$4520007 & $65.526284$ & $45.333530$ & $3363$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J04224583$+$5639474 & $65.690970$ & $56.663181$ & $3687$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J04234272$+$5605429 & $65.928032$ & $56.095268$ & $3253$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J04301819$+$3601341 & $67.575800$ & $36.026157$ & $3596$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J04303552$+$4626098 & $67.648033$ & $46.436077$ & $2950$ & $3000$ & $-0.5$ & $5.0$ & $<8.0$\\
J04312929$+$4141107 & $67.872049$ & $41.686321$ & $3212$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J04314295$+$3552302 & $67.928972$ & $35.875080$ & $3316$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J04325303$+$3608084 & $68.220973$ & $36.135681$ & $3763$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J04331975$+$4719064 & $68.332292$ & $47.318455$ & $3319$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J04341592$+$3449315 & $68.566362$ & $34.825443$ & $3539$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J04351236$+$5821100 & $68.801504$ & $58.352779$ & $3356$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J04351537$+$4727272 & $68.814077$ & $47.457561$ & $3006$ & $3100$ & $-0.5$ & $5.5$ & $<8.0$\\
J04360976$+$4059136 & $69.040703$ & $40.987129$ & $3428$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J04370219$+$4230427 & $69.259135$ & $42.511875$ & $3145$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J04371030$+$4703549 & $69.292935$ & $47.065273$ & $3564$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J04373881$+$4650216 & $69.411745$ & $46.839359$ & $3408$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J04393348$+$4132488 & $69.889512$ & $41.546909$ & $3104$ & $3100$ & $-0.0$ & $5.0$ & $<8.0$\\
J04414771$+$4149500 & $70.448829$ & $41.830559$ & $3204$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J04421031$+$3803170 & $70.542978$ & $38.054749$ & $3272$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J04421603$+$5742275 & $70.566824$ & $57.707649$ & $3855$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J04422854$+$5818015 & $70.618956$ & $58.300430$ & $3274$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J04442617$+$5840464 & $71.109058$ & $58.679573$ & $3535$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J04471285$+$3957231 & $71.803554$ & $39.956429$ & $2920$ & $2900$ & $-0.0$ & $5.5$ & $<8.0$\\
J04480390$+$5718092 & $72.016273$ & $57.302570$ & $3218$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J04480517$+$3732402 & $72.021548$ & $37.544518$ & $3163$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J04483289$+$5003109 & $72.137081$ & $50.053028$ & $3436$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J04515998$+$5749173 & $72.999955$ & $57.821499$ & $2824$ & $2900$ & $-0.0$ & $5.5$ & $<8.0$\\
J04531256$+$3830323 & $73.302365$ & $38.508999$ & $3640$ & $3600$ & $-1.0$ & $4.5$ & $<8.0$\\
J04542406$+$3830436 & $73.600261$ & $38.512138$ & $3007$ & $3100$ & $-0.5$ & $5.5$ & $<8.0$\\
J04572720$+$5038596 & $74.363345$ & $50.649906$ & $3318$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J04584599$+$5056378 & $74.691634$ & $50.943859$ & $3807$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J04592075$+$3434124 & $74.836459$ & $34.570118$ & $3772$ & $3800$ & $+0.5$ & $5.0$ & $<8.0$\\
J04592826$+$4922300 & $74.867753$ & $49.375004$ & $3309$ & $3300$ & $-0.5$ & $4.5$ & $<8.0$\\
J05011792$+$4204125 & $75.324677$ & $42.070148$ & $3656$ & $3700$ & $+0.5$ & $5.0$ & $<8.0$\\
J05011802$+$2237015 & $75.325112$ & $22.617104$ & $3019$ & $3000$ & $-0.0$ & $5.5$ & $<8.0$\\
J05014512$+$5039319 & $75.438022$ & $50.658867$ & $3605$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J05014944$+$2127375 & $75.456010$ & $21.460436$ & $3319$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J05030563$+$2122362 & $75.773472$ & $21.376726$ & $3094$ & $3100$ & $+0.5$ & $5.5$ & $21.7\pm1.5$\\
J05031170$+$4652485 & $75.798765$ & $46.880161$ & $3313$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J05052561$+$4552058 & $76.356738$ & $45.868279$ & $3463$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J05053461$+$4648017 & $76.394216$ & $46.800491$ & $2632$ & $2600$ & $-0.0$ & $5.5$ & $<8.0$\\
J05062444$+$2230199 & $76.601841$ & $22.505548$ & $3003$ & $3000$ & $-0.0$ & $5.0$ & $<8.0$\\
J05104796$+$2410125 & $77.699863$ & $24.170149$ & $3242$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J05160907$+$2305202 & $79.037795$ & $23.088959$ & $3437$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J05171875$+$2320177 & $79.328147$ & $23.338255$ & $3332$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J05181814$+$2426180 & $79.575622$ & $24.438339$ & $3304$ & $3300$ & $-0.5$ & $5.0$ & $<8.0$\\
J05210188$+$3425119 & $80.257859$ & $34.419991$ & $3144$ & $3100$ & $+0.5$ & $5.0$ & $<8.0$\\
J05243459$+$2940434 & $81.144127$ & $29.678741$ & $3249$ & $3200$ & $-0.0$ & $4.5$ & $14.1\pm1.6$\\
J05255532$+$3528438 & $81.480519$ & $35.478859$ & $3097$ & $3000$ & $-0.0$ & $5.0$ & $<8.0$\\
J05282466$+$3944589 & $82.102786$ & $39.749706$ & $3661$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J05292369$+$2619582 & $82.348730$ & $26.332836$ & $3699$ & $3800$ & $-0.0$ & $5.0$ & $<8.0$\\
J05292729$+$2724457 & $82.363726$ & $27.412695$ & $3911$ & $4000$ & $-0.0$ & $4.5$ & $<8.0$\\
J05313118$+$3916413 & $82.879940$ & $39.278164$ & $3732$ & $3700$ & $-0.5$ & $4.5$ & $9.42\pm1.5$\\
J05313731$+$4128000 & $82.905464$ & $41.466667$ & $3622$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J05320969$+$2754534 & $83.040394$ & $27.914845$ & $2865$ & $2900$ & $-0.0$ & $5.5$ & $8.36\pm1.7$\\
J05325989$+$2608271 & $83.249549$ & $26.140879$ & $3342$ & $3400$ & $+0.5$ & $5.5$ & $47.7\pm2.3$\\
J05343882$+$2646318 & $83.661783$ & $26.775509$ & $3303$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J05344102$+$2345373 & $83.670946$ & $23.760366$ & $3551$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J05352750$+$2558217 & $83.864597$ & $25.972712$ & $3552$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J05392474$+$4038437 & $84.853102$ & $40.645485$ & $2627$ & $2600$ & $-0.0$ & $5.0$ & $<8.0$\\
J05402570$+$2448090 & $85.107108$ & $24.802505$ & $2799$ & $2800$ & $-0.0$ & $5.0$ & $25.9\pm1.7$\\
J05405944$+$4451075 & $85.247707$ & $44.852085$ & $3795$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J05424060$+$6134403 & $85.669180$ & $61.577881$ & $3153$ & $3100$ & $+0.5$ & $5.0$ & $<8.0$\\
J05425532$+$2032498 & $85.730537$ & $20.547194$ & $3729$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J05430330$+$2307473 & $85.763789$ & $23.129816$ & $3350$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J05431104$+$2429510 & $85.796016$ & $24.497520$ & $3230$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J05433934$+$1212368 & $85.913952$ & $12.210247$ & $3550$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J05444137$+$2120494 & $86.172402$ & $21.347078$ & $3335$ & $3300$ & $-0.5$ & $4.5$ & $<8.0$\\
J05470652$+$2913272 & $86.777205$ & $29.224243$ & $3396$ & $3300$ & $+0.5$ & $4.5$ & $<8.0$\\
J05470907$-$0512106 & $86.787800$ & $-5.2029690$ & $3149$ & $3100$ & $+0.5$ & $5.0$ & $<8.0$\\
J05471262$+$3452336 & $86.802622$ & $34.876019$ & $3298$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J05483220$+$2119180 & $87.134207$ & $21.321693$ & $3334$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J05483253$+$2117577 & $87.135550$ & $21.299368$ & $3789$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J05504636$+$1107476 & $87.693196$ & $11.129915$ & $3482$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J05513253$+$1148359 & $87.885556$ & $11.809979$ & $3585$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J05531424$+$1742115 & $88.309373$ & $17.703199$ & $3288$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J05571864$+$1708299 & $89.327684$ & $17.141666$ & $3180$ & $3200$ & $-0.5$ & $4.5$ & $<8.0$\\
J05580690$+$1557564 & $89.528757$ & $15.965684$ & $3418$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J05593985$+$3040401 & $89.916050$ & $30.677822$ & $3840$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J06000658$+$2936555 & $90.027432$ & $29.615433$ & $3185$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J06025298$+$3129415 & $90.720790$ & $31.494867$ & $3259$ & $3200$ & $-0.5$ & $4.5$ & $<8.0$\\
J06043950$+$2753529 & $91.164594$ & $27.898035$ & $3560$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J06070493$+$1403109 & $91.770553$ & $14.053038$ & $3246$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J06075349$+$2746207 & $91.972899$ & $27.772421$ & $3788$ & $3900$ & $-0.0$ & $5.0$ & $<8.0$\\
J06081784$+$0934466 & $92.074349$ & $9.5796210$ & $3199$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J06090208$+$2633257 & $92.258676$ & $26.557154$ & $3560$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J06092734$+$1116298 & $92.363931$ & $11.274962$ & $3624$ & $3600$ & $-0.5$ & $4.5$ & $8.19\pm1.8$\\
J06093542$+$2816546 & $92.397587$ & $28.281841$ & $3121$ & $3000$ & $-0.0$ & $5.0$ & $<8.0$\\
J06101073$+$1032302 & $92.544712$ & $10.541748$ & $3877$ & $3900$ & $-0.5$ & $4.5$ & $<8.0$\\
J06101085$+$1119546 & $92.545220$ & $11.331850$ & $2999$ & $3100$ & $-0.5$ & $5.5$ & $<8.0$\\
J06102756$+$2759447 & $92.614863$ & $27.995758$ & $3732$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J06112610$+$1032599 & $92.858786$ & $10.549991$ & $3713$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J06112868$+$1008375 & $92.869522$ & $10.143766$ & $3040$ & $3100$ & $+0.5$ & $5.5$ & $<8.0$\\
J06115599$+$3325505 & $92.983296$ & $33.430714$ & $3198$ & $3200$ & $+0.5$ & $5.5$ & $12.5\pm1.7$\\
J06125467$+$1006313 & $93.227797$ & $10.108707$ & $3299$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J06132113$+$2835295 & $93.338059$ & $28.591534$ & $3553$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J06134814$+$2335489 & $93.450607$ & $23.596943$ & $3080$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J06134854$+$2647211 & $93.452287$ & $26.789215$ & $3826$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J06150622$+$3248010 & $93.775926$ & $32.800289$ & $3282$ & $3300$ & $-0.5$ & $4.5$ & $<8.0$\\
J06161499$+$2754094 & $94.062485$ & $27.902634$ & $3547$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J06195743$+$2022197 & $94.989307$ & $20.372139$ & $3010$ & $3100$ & $-0.0$ & $5.0$ & $28.9\pm1.6$\\
J06205178$+$3145134 & $95.215783$ & $31.753725$ & $3109$ & $3100$ & $+0.5$ & $5.5$ & $<8.0$\\
J06213640$+$3222390 & $95.401669$ & $32.377506$ & $3009$ & $3100$ & $-0.5$ & $5.5$ & $<8.0$\\
J06213904$+$3231006 & $95.412706$ & $32.516853$ & $3356$ & $3300$ & $-0.5$ & $5.0$ & $<8.0$\\
J06234645$+$0502411 & $95.943550$ & $5.0447640$ & $3861$ & $3900$ & $+0.5$ & $5.0$ & $<8.0$\\
J06270211$+$0309473 & $96.758825$ & $3.1631440$ & $3642$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J06272815$+$2129225 & $96.867315$ & $21.489595$ & $3043$ & $3000$ & $-0.0$ & $5.0$ & $11.4\pm1.6$\\
J06273672$+$0918088 & $96.903008$ & $9.3024590$ & $3664$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J06274397$+$0923541 & $96.933209$ & $9.3983620$ & $3611$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J06293433$+$1742419 & $97.393073$ & $17.711651$ & $3081$ & $3000$ & $-0.0$ & $5.0$ & $<8.0$\\
J06295663$+$0934185 & $97.485987$ & $9.5718210$ & $3312$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J06312373$+$0036445 & $97.848903$ & $0.61236300$ & $3673$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J06320207$+$3431132 & $98.008631$ & $34.520336$ & $3260$ & $3200$ & $+0.5$ & $5.0$ & $<8.0$\\
J06322227$+$0044222 & $98.092822$ & $0.73950000$ & $3562$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J06362535$+$1830520 & $99.105655$ & $18.514462$ & $3283$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J06370004$+$1515162 & $99.250177$ & $15.254525$ & $3647$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J06375540$+$0858594 & $99.480852$ & $8.9831830$ & $3247$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J06383035$+$1455167 & $99.626484$ & $14.921312$ & $3399$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J06405199$+$1543220 & $100.21666$ & $15.722780$ & $3372$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J06421118$+$0334527 & $100.54659$ & $3.5813060$ & $3437$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J06434596$+$1410450 & $100.94151$ & $14.179173$ & $3663$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J06464003$+$0109157 & $101.66680$ & $1.1543710$ & $3842$ & $4000$ & $-0.5$ & $4.5$ & $32.5\pm1.9$\\
J06473451$+$0748593 & $101.89379$ & $7.8164740$ & $3153$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J06481555$+$0326243 & $102.06481$ & $3.4400940$ & $2786$ & $2800$ & $-0.0$ & $5.5$ & $8.92\pm1.6$\\
J06503126$-$0938441 & $102.63028$ & $-9.6455880$ & $3571$ & $3600$ & $-1.0$ & $4.5$ & $<8.0$\\
J06505947$-$0910506 & $102.74783$ & $-9.1807240$ & $3397$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J06513673$+$2023264 & $102.90308$ & $20.390667$ & $3481$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J06542485$+$1653352 & $103.60357$ & $16.893133$ & $3652$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J06543764$+$1708058 & $103.65684$ & $17.134947$ & $3408$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J06561894$-$0835461 & $104.07894$ & $-8.5961490$ & $3343$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J06572462$+$0651440 & $104.35260$ & $6.8622410$ & $3218$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J07015902$+$0456273 & $105.49594$ & $4.9409210$ & $3197$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J07092008$+$0017352 & $107.33370$ & $0.29313200$ & $3402$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J07171706$-$0501031 & $109.32108$ & $-5.0175380$ & $3160$ & $3200$ & $-0.0$ & $5.0$ & $27.9\pm1.6$\\
J07355815$+$7832528 & $113.99229$ & $78.548027$ & $3476$ & $3500$ & $-0.0$ & $5.0$ & $<8.0$\\
J07404251$+$6643075 & $115.17714$ & $66.718765$ & $3851$ & $3800$ & $-0.0$ & $4.5$ & $11.4\pm1.9$\\
J07404603$+$3758253 & $115.19180$ & $37.973721$ & $3166$ & $3000$ & $+0.5$ & $4.5$ & $<8.0$\\
J07421457$+$7949418 & $115.56071$ & $79.828278$ & $3266$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J07431638$+$6642456 & $115.81828$ & $66.712685$ & $3532$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J07444028$+$7946423 & $116.16787$ & $79.778435$ & $3838$ & $3800$ & $-0.0$ & $4.5$ & $52.8\pm2.6$\\
J07454991$+$3716280 & $116.45799$ & $37.274448$ & $3253$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J07461563$+$5359345 & $116.56516$ & $53.992924$ & $3268$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J07492701$+$7752423 & $117.36257$ & $77.878433$ & $3308$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J07551206$+$5257540 & $118.80027$ & $52.965000$ & $3353$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J07560879$+$4110179 & $119.03665$ & $41.171650$ & $3798$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J07562017$+$3935254 & $119.08407$ & $39.590393$ & $3540$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J07563272$+$4011016 & $119.13636$ & $40.183796$ & $3596$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J07573472$+$3940005 & $119.39471$ & $39.666813$ & $3781$ & $3900$ & $-0.5$ & $4.5$ & $<8.0$\\
J07592679$+$4118003 & $119.86166$ & $41.300095$ & $3547$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J08025304$+$4012352 & $120.72101$ & $40.209805$ & $3369$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J08070156$+$7832436 & $121.75652$ & $78.545464$ & $3296$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J08074747$+$4013412 & $121.94782$ & $40.228127$ & $3563$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J08100405$+$3220142 & $122.51689$ & $32.337296$ & $3503$ & $3500$ & $-0.0$ & $4.5$ & $17.4\pm1.5$\\
J08103429$-$1348514 & $122.64288$ & $-13.814298$ & $3582$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J08122671$+$2745298 & $123.11131$ & $27.758286$ & $3348$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J08140773$+$2703384 & $123.53221$ & $27.060671$ & $3535$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J08151813$+$7946294 & $123.82555$ & $79.774849$ & $3644$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J08155393$+$3136392 & $123.97472$ & $31.610901$ & $3865$ & $3900$ & $-0.0$ & $4.5$ & $23.9\pm1.6$\\
J08160527$+$3028386 & $124.02197$ & $30.477396$ & $3063$ & $3000$ & $+0.5$ & $5.5$ & $<8.0$\\
J08175130$+$3107455 & $124.46376$ & $31.129322$ & $3792$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J08185024$+$7843250 & $124.70935$ & $78.723625$ & $3481$ & $3500$ & $-0.0$ & $5.0$ & $<8.0$\\
J08370799$+$1507475 & $129.28330$ & $15.129878$ & $3484$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J08501918$+$1056436 & $132.57994$ & $10.945469$ & $3171$ & $3200$ & $-0.0$ & $5.0$ & $15.8\pm1.5$\\
J08505983$+$1130493 & $132.74930$ & $11.513719$ & $3103$ & $3100$ & $-0.0$ & $5.0$ & $<8.0$\\
J08535174$+$0318422 & $133.46560$ & $3.3117470$ & $3556$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J08584396$+$3727389 & $134.68318$ & $37.460819$ & $3436$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J08595755$+$0417552 & $134.98979$ & $4.2986870$ & $3758$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J09005033$+$0514293 & $135.20971$ & $5.2414950$ & $3392$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J09010280$+$0237517 & $135.26170$ & $2.6310440$ & $3380$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J09022952$+$0417072 & $135.62304$ & $4.2853460$ & $3334$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J09031291$+$3739077 & $135.80381$ & $37.652142$ & $3078$ & $3000$ & $-0.0$ & $5.0$ & $<8.0$\\
J09285333$-$0722148 & $142.22224$ & $-7.3707930$ & $3437$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J09301445$+$2630250 & $142.56023$ & $26.506958$ & $3439$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J09321296$+$2745465 & $143.05401$ & $27.762943$ & $3142$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J09391173$+$3837561 & $144.79891$ & $38.632263$ & $3051$ & $3000$ & $-0.0$ & $5.0$ & $10.8\pm1.6$\\
J09422327$+$5559015 & $145.59698$ & $55.983776$ & $3390$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J10162955$+$0318375 & $154.12313$ & $3.3104190$ & $3355$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J10164852$+$0041408 & $154.20220$ & $0.69469400$ & $3150$ & $3100$ & $+0.5$ & $5.0$ & $<8.0$\\
J10294592$+$2845089 & $157.44134$ & $28.752493$ & $3412$ & $3600$ & $+0.5$ & $5.0$ & $<8.0$\\
J10304397$+$1624207 & $157.68321$ & $16.405760$ & $3104$ & $3200$ & $-0.0$ & $5.5$ & $<8.0$\\
J10305410$+$3008526 & $157.72544$ & $30.147951$ & $3692$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J10305842$+$2937180 & $157.74342$ & $29.621675$ & $3363$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J10311010$+$3517565 & $157.79211$ & $35.299034$ & $3287$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J10312674$+$3436011 & $157.86142$ & $34.600319$ & $3438$ & $3500$ & $+0.5$ & $5.0$ & $<8.0$\\
J10330667$+$2837490 & $158.27782$ & $28.630287$ & $3366$ & $3400$ & $+0.5$ & $5.5$ & $<8.0$\\
J10331367$+$3409120 & $158.30698$ & $34.153358$ & $3667$ & $3500$ & $+0.5$ & $5.0$ & $11.7\pm1.5$\\
J10345281$+$3911043 & $158.72005$ & $39.184532$ & $3323$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J10355725$+$2853316 & $158.98856$ & $28.892134$ & $3442$ & $3500$ & $-0.0$ & $5.0$ & $<8.0$\\
J10361794$+$2844471 & $159.07477$ & $28.746441$ & $3929$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J10371967$+$3534363 & $159.33199$ & $35.576767$ & $3999$ & $4000$ & $-0.0$ & $4.5$ & $<8.0$\\
J10373423$+$2959387 & $159.39264$ & $29.994093$ & $3214$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J10381018$+$1938087 & $159.54244$ & $19.635754$ & $3443$ & $3500$ & $-0.0$ & $5.0$ & $<8.0$\\
J10383323$+$3529492 & $159.63848$ & $35.497002$ & $3536$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J10385685$+$2505402 & $159.73692$ & $25.094526$ & $3624$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J10391962$+$3044566 & $159.83178$ & $30.749065$ & $3545$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J10393463$+$3809488 & $159.89430$ & $38.163570$ & $3244$ & $3200$ & $+0.5$ & $5.0$ & $<8.0$\\
J10394863$+$3034105 & $159.95265$ & $30.569605$ & $3343$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J10401225$+$3510463 & $160.05105$ & $35.179550$ & $3505$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J10420683$+$1937123 & $160.52848$ & $19.620090$ & $3388$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J10423925$+$1944404 & $160.66354$ & $19.744581$ & $3350$ & $3300$ & $-0.0$ & $4.5$ & $28.7\pm1.5$\\
J10441137$+$4500152 & $161.04738$ & $45.004227$ & $3818$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J10464178$+$1924065 & $161.67409$ & $19.401825$ & $3357$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J10473327$+$2007406 & $161.88866$ & $20.127953$ & $3432$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J10475231$+$2020315 & $161.96796$ & $20.342108$ & $3663$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J10482532$+$4320339 & $162.10553$ & $43.342770$ & $3409$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J10483255$+$1909022 & $162.13566$ & $19.150629$ & $3413$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J10510361$+$1458198 & $162.76507$ & $14.972180$ & $3242$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J10524422$+$1440483 & $163.18427$ & $14.680103$ & $3657$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J10533037$+$4457504 & $163.37655$ & $44.964012$ & $3699$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J10540048$+$1606059 & $163.50201$ & $16.101650$ & $3024$ & $3000$ & $-0.0$ & $5.5$ & $<8.0$\\
J10550664$+$1532443 & $163.77769$ & $15.545649$ & $3986$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J10560279$+$4858238 & $164.01165$ & $48.973282$ & $3945$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J10562960$+$4858264 & $164.12337$ & $48.974018$ & $3982$ & $4000$ & $+0.5$ & $5.0$ & $<8.0$\\
J10572599$+$4923562 & $164.35832$ & $49.398972$ & $3619$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J11014478$+$1227162 & $165.43659$ & $12.454500$ & $3419$ & $3400$ & $-0.0$ & $4.5$ & $9.30\pm1.6$\\
J11034699$+$4932532 & $165.94579$ & $49.548138$ & $3314$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J11123132$+$0627518 & $168.13051$ & $6.4644150$ & $3373$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J11144514$+$0035134 & $168.68811$ & $0.58707100$ & $3387$ & $3400$ & $-0.5$ & $5.0$ & $<8.0$\\
J11173203$+$0013050 & $169.38349$ & $0.21806700$ & $3464$ & $3500$ & $-0.0$ & $5.0$ & $<8.0$\\
J11323130$+$0334390 & $173.13044$ & $3.5775070$ & $3336$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J11323938$+$0513167 & $173.16410$ & $5.2213270$ & $3806$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J11353571$+$0414146 & $173.89882$ & $4.2374150$ & $3557$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J11354036$+$0457295 & $173.91820$ & $4.9582110$ & $3421$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J11401965$+$2552492 & $175.08188$ & $25.880356$ & $3671$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J11434490$+$0200430 & $175.93710$ & $2.0119600$ & $3426$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J11450282$+$2601155 & $176.26178$ & $26.020977$ & $3319$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J11463262$+$0130524 & $176.63592$ & $1.5145820$ & $3045$ & $3000$ & $-0.0$ & $5.0$ & $<8.0$\\
J11463674$+$2719315 & $176.65309$ & $27.325417$ & $3388$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J11474074$+$0015201 & $176.91977$ & $0.25560400$ & $3311$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J11480063$+$3505146 & $177.00265$ & $35.087391$ & $3672$ & $3700$ & $+0.5$ & $5.0$ & $<8.0$\\
J11501565$+$2625126 & $177.56521$ & $26.420174$ & $3466$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J11511794$+$1829229 & $177.82478$ & $18.489714$ & $3422$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J11512352$+$5411127 & $177.84800$ & $54.186882$ & $3315$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J11521203$+$2032148 & $178.05016$ & $20.537460$ & $3857$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J11530522$+$1855480 & $178.27179$ & $18.930019$ & $3831$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J11550416$+$3526308 & $178.76735$ & $35.441910$ & $3580$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J11572662$+$3425414 & $179.36096$ & $34.428169$ & $3226$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J11580290$+$2013015 & $179.51209$ & $20.217106$ & $3377$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J11593840$+$1545481 & $179.91001$ & $15.763388$ & $3434$ & $3600$ & $+0.5$ & $5.5$ & $<8.0$\\
J12005016$+$1938424 & $180.20901$ & $19.645123$ & $3522$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J12033893$+$1527533 & $180.91224$ & $15.464808$ & $3378$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J12045611$+$1728119 & $181.23380$ & $17.469975$ & $3379$ & $3300$ & $-0.0$ & $5.0$ & $17.0\pm1.6$\\
J12045619$+$1757409 & $181.23414$ & $17.961363$ & $3238$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J12054224$+$1844354 & $181.42604$ & $18.743189$ & $3336$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J12070374$+$0012509 & $181.76562$ & $0.21415900$ & $3609$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J12081374$+$1747306 & $182.05728$ & $17.791861$ & $3074$ & $3200$ & $-0.5$ & $5.5$ & $<8.0$\\
J12081818$+$4027012 & $182.07579$ & $40.450340$ & $3840$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J12082601$+$4022490 & $182.10840$ & $40.380280$ & $3747$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J12102152$+$4026185 & $182.58967$ & $40.438484$ & $3653$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J12102884$+$3950539 & $182.62017$ & $39.848328$ & $3426$ & $3400$ & $-0.0$ & $5.0$ & $8.58\pm2.6$\\
J12105688$+$4103275 & $182.73702$ & $41.057655$ & $3837$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J12110303$+$4043482 & $182.76263$ & $40.730057$ & $3435$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J12110614$+$1846153 & $182.77561$ & $18.770939$ & $3327$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J12121359$+$1356531 & $183.05663$ & $13.948107$ & $3220$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J12122940$+$3940281 & $183.12250$ & $39.674492$ & $3728$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J12135956$+$3910101 & $183.49819$ & $39.169487$ & $3652$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J12140441$+$1526225 & $183.51839$ & $15.439595$ & $3734$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J12152838$+$3911145 & $183.86826$ & $39.187374$ & $3721$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J12153222$+$1515555 & $183.88425$ & $15.265443$ & $3323$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J12173762$+$1252395 & $184.40678$ & $12.877663$ & $3461$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J12200119$+$2633419 & $185.00498$ & $26.561646$ & $3251$ & $3200$ & $-0.0$ & $4.5$ & $8.07\pm1.6$\\
J12201448$+$2526072 & $185.06035$ & $25.435360$ & $3369$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J12203573$+$4104277 & $185.14888$ & $41.074387$ & $3469$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J12211807$+$1526341 & $185.32530$ & $15.442816$ & $3405$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J12212146$+$5745089 & $185.33946$ & $57.752480$ & $3655$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J12213891$+$3956445 & $185.41213$ & $39.945698$ & $3549$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J12222073$+$0011020 & $185.58640$ & $0.18390900$ & $3064$ & $3000$ & $+0.5$ & $4.5$ & $<8.0$\\
J12223238$+$5730387 & $185.63496$ & $57.510769$ & $3431$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J12232063$+$2529441 & $185.83597$ & $25.495592$ & $3399$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J12241121$+$2653166 & $186.04672$ & $26.887962$ & $3826$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J12243585$+$0001106 & $186.14941$ & $0.019618000$ & $3256$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J12244171$+$1405391 & $186.17381$ & $14.094218$ & $3326$ & $3400$ & $+0.5$ & $5.5$ & $<8.0$\\
J12251686$+$5531004 & $186.32028$ & $55.516804$ & $3472$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J12253159$+$0011354 & $186.38165$ & $0.19318600$ & $3267$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J12265737$+$2700536 & $186.73904$ & $27.014906$ & $3143$ & $3100$ & $-0.0$ & $5.0$ & $9.27\pm1.4$\\
J12271328$+$5705444 & $186.80534$ & $57.095684$ & $3596$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J12281495$+$5526169 & $187.06230$ & $55.438030$ & $3669$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J12285007$+$2717414 & $187.20865$ & $27.294849$ & $3994$ & $4000$ & $-0.0$ & $4.5$ & $<8.0$\\
J12301148$+$5555229 & $187.54784$ & $55.923038$ & $3580$ & $3500$ & $-0.5$ & $4.5$ & $8.51\pm1.8$\\
J12304702$+$2603294 & $187.69595$ & $26.058172$ & $3043$ & $3000$ & $-0.0$ & $5.0$ & $<8.0$\\
J12311836$+$5642299 & $187.82652$ & $56.708328$ & $3553$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J12330155$+$5738113 & $188.25649$ & $57.636497$ & $3560$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J12333581$+$5551297 & $188.39923$ & $55.858273$ & $3603$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J12442074$-$0150374 & $191.08644$ & $-1.8437330$ & $3334$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J12505082$+$1301468 & $192.71179$ & $13.029672$ & $3393$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J12514238$+$4144060 & $192.92659$ & $41.735027$ & $3462$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J12523581$+$4320484 & $193.14923$ & $43.346783$ & $3974$ & $4000$ & $-0.0$ & $4.5$ & $<8.0$\\
J12544133$+$4323125 & $193.67224$ & $43.386822$ & $3228$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J12573249$+$4057012 & $194.38541$ & $40.950356$ & $3644$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J12592744$+$5633464 & $194.86437$ & $56.562904$ & $3415$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J13024751$+$4131098 & $195.69799$ & $41.519409$ & $3498$ & $3500$ & $+0.5$ & $5.0$ & $<8.0$\\
J13075012$+$1717471 & $196.95887$ & $17.296432$ & $3245$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J13085059$+$1622039 & $197.21079$ & $16.367750$ & $3439$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J13085124$-$0131075 & $197.21351$ & $-1.5187690$ & $3498$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J13095556$+$1438595 & $197.48153$ & $14.649865$ & $3593$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J13104586$+$7137564 & $197.69108$ & $71.632339$ & $3236$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J13141940$+$1256164 & $198.58086$ & $12.937913$ & $3360$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J13142039$+$1320011 & $198.58497$ & $13.333663$ & $2789$ & $2900$ & $-0.0$ & $5.5$ & $49.1\pm1.9$\\
J13160127$+$1415504 & $199.00531$ & $14.264018$ & $3785$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J13190031$+$1236476 & $199.75132$ & $12.613233$ & $3419$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J13194909$+$1313552 & $199.95455$ & $13.232025$ & $3442$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J13200576$+$1339093 & $200.02402$ & $13.652610$ & $3315$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J13201255$-$0140407 & $200.05231$ & $-1.6779740$ & $3376$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J13202492$-$0139266 & $200.10386$ & $-1.6574080$ & $3680$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J13243627$+$1308050 & $201.15115$ & $13.134744$ & $3719$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J13265928$+$3840199 & $201.74702$ & $38.672207$ & $3296$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J13273648$+$7310418 & $201.90201$ & $73.178299$ & $3198$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J13273827$+$5628102 & $201.90948$ & $56.469501$ & $3410$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J13275779$+$4001237 & $201.99083$ & $40.023273$ & $3264$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J13284371$+$3823292 & $202.18214$ & $38.391468$ & $3388$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J13313770$+$3821415 & $202.90712$ & $38.361534$ & $3294$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J13315838$+$5443452 & $202.99329$ & $54.729248$ & $3663$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J13331747$+$3833314 & $203.32283$ & $38.558735$ & $3205$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J13332256$+$3620352 & $203.34402$ & $36.343117$ & $3959$ & $4000$ & $-0.0$ & $4.5$ & $<8.0$\\
J13335128$+$5647303 & $203.46369$ & $56.791759$ & $3328$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J13402618$+$5448480 & $205.10911$ & $54.813354$ & $3248$ & $3200$ & $+0.5$ & $5.0$ & $<8.0$\\
J13421941$+$1847193 & $205.58089$ & $18.788717$ & $3804$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J13451104$+$2852012 & $206.29603$ & $28.867016$ & $3409$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J13455527$+$2723131 & $206.48032$ & $27.386990$ & $3318$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J13462582$+$0102336 & $206.60760$ & $1.0426940$ & $3017$ & $3100$ & $-0.0$ & $5.5$ & $8.93\pm1.6$\\
J13462703$+$1707100 & $206.61263$ & $17.119467$ & $3662$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J13490570$+$1900101 & $207.27376$ & $19.002823$ & $3552$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J13491436$+$2637457 & $207.30984$ & $26.629383$ & $3263$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J13495762$+$1746261 & $207.49009$ & $17.773920$ & $3440$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J13525797$+$3331361 & $208.24156$ & $33.526699$ & $3473$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J13532486$+$3418182 & $208.35358$ & $34.305069$ & $3324$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J13532938$+$4416109 & $208.37242$ & $44.269707$ & $3220$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J13542316$+$2543152 & $208.59652$ & $25.720890$ & $3191$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J13564148$+$4342587 & $209.17285$ & $43.716324$ & $2626$ & $2600$ & $-0.0$ & $5.0$ & $13.5\pm1.6$\\
J13565257$+$3407095 & $209.21906$ & $34.119320$ & $3344$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J13570155$+$2534378 & $209.25648$ & $25.577177$ & $3735$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J13570533$+$2638437 & $209.27223$ & $26.645475$ & $3320$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J13572571$+$3400176 & $209.35713$ & $34.004890$ & $3463$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J14001449$+$2446001 & $210.06039$ & $24.766703$ & $3802$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J14010995$+$2621429 & $210.29147$ & $26.361925$ & $3868$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J14011705$+$5431528 & $210.32106$ & $54.531342$ & $3112$ & $3100$ & $+0.5$ & $5.5$ & $16.0\pm1.5$\\
J14022009$+$0105058 & $210.58372$ & $1.0849540$ & $3312$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J14022155$+$2517517 & $210.58982$ & $25.297712$ & $3769$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J14035430$+$3008026 & $210.97626$ & $30.134077$ & $3413$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J14044784$+$5237559 & $211.19935$ & $52.632206$ & $3444$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J14045583$+$0157230 & $211.23263$ & $1.9564070$ & $3695$ & $3600$ & $+0.5$ & $5.0$ & $<8.0$\\
J14081562$+$5236281 & $212.06510$ & $52.607822$ & $3153$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J14085680$+$5253324 & $212.23668$ & $52.892334$ & $3342$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J14130286$+$0506321 & $213.26192$ & $5.1089380$ & $3395$ & $3400$ & $+0.5$ & $5.5$ & $<8.0$\\
J14152232$+$5324435 & $213.84302$ & $53.412086$ & $3296$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J14173915$+$0624144 & $214.41315$ & $6.4040050$ & $3315$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J14212272$+$0425137 & $215.34468$ & $4.4204970$ & $3533$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J14213453$+$0431315 & $215.39390$ & $4.5254260$ & $3490$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J14320849$+$0811313 & $218.03541$ & $8.1920370$ & $2948$ & $3000$ & $-0.0$ & $5.5$ & $8.49\pm1.5$\\
J14321453$+$4939058 & $218.06056$ & $49.651615$ & $3239$ & $3300$ & $-0.5$ & $4.5$ & $<8.0$\\
J14323211$+$5104591 & $218.13381$ & $51.083107$ & $3003$ & $3100$ & $-0.5$ & $5.5$ & $<8.0$\\
J14333756$+$0852369 & $218.40652$ & $8.8769290$ & $3293$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J14333985$+$0920094 & $218.41606$ & $9.3359630$ & $3384$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J14351526$+$5023415 & $218.81362$ & $50.394871$ & $3420$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J14351820$+$0959247 & $218.82587$ & $9.9902150$ & $3425$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J14371551$+$0926211 & $219.31463$ & $9.4392170$ & $3275$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J14385800$+$1327388 & $219.74169$ & $13.460784$ & $3696$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J14413024$+$1337362 & $220.37604$ & $13.626726$ & $3763$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J14431906$+$1120548 & $220.82944$ & $11.348572$ & $3479$ & $3500$ & $-0.0$ & $5.0$ & $<8.0$\\
J14432141$+$4514097 & $220.83925$ & $45.236046$ & $3504$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J14532894$+$1716317 & $223.37060$ & $17.275492$ & $3461$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J14535251$+$1739448 & $223.46882$ & $17.662457$ & $3765$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J14540912$+$4135008 & $223.53803$ & $41.583557$ & $3513$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J14542360$+$4041246 & $223.59835$ & $40.690189$ & $3676$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J14544041$+$1634428 & $223.66841$ & $16.578566$ & $3656$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J14545496$+$4108480 & $223.72903$ & $41.146690$ & $3238$ & $3300$ & $+0.5$ & $5.5$ & $44.1\pm1.6$\\
J14545704$+$3714558 & $223.73769$ & $37.248859$ & $3564$ & $3600$ & $+0.5$ & $5.0$ & $<8.0$\\
J14551346$+$4128494 & $223.80611$ & $41.480396$ & $3560$ & $3500$ & $+0.5$ & $5.5$ & $<8.0$\\
J14562518$+$1655399 & $224.10492$ & $16.927769$ & $3411$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J14563077$+$4115236 & $224.12822$ & $41.256561$ & $3651$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J14573227$+$3123446 & $224.38448$ & $31.395733$ & $3884$ & $3900$ & $-0.5$ & $4.5$ & $<8.0$\\
J15024283$+$3211141 & $225.67849$ & $32.187275$ & $3549$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J15035753$+$4242155 & $225.98975$ & $42.704315$ & $3225$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J15041817$+$3053139 & $226.07574$ & $30.887222$ & $3321$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J15043302$+$2056136 & $226.13759$ & $20.937136$ & $3641$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J15045746$+$3715425 & $226.23946$ & $37.261806$ & $3482$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J15090689$+$3254449 & $227.27872$ & $32.912495$ & $3432$ & $3500$ & $+0.5$ & $5.5$ & $<8.0$\\
J15165576$-$0037116 & $229.23237$ & $-0.61989700$ & $3180$ & $3300$ & $-0.5$ & $5.5$ & $<8.0$\\
J15262530$+$3758599 & $231.60546$ & $37.983307$ & $3209$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J15272423$+$3714148 & $231.85096$ & $37.237446$ & $3141$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J15281240$+$4340086 & $232.05168$ & $43.669071$ & $3353$ & $3300$ & $-0.0$ & $5.0$ & $8.16\pm1.6$\\
J16084780$+$2219306 & $242.19919$ & $22.325188$ & $3270$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J16193140$+$5206469 & $244.88084$ & $52.113033$ & $3298$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J16204000$+$8624065 & $245.16669$ & $86.401833$ & $3507$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J16261429$+$8558497 & $246.55955$ & $85.980499$ & $3174$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J16340737$+$0038043 & $248.53075$ & $0.63454700$ & $3390$ & $3300$ & $-0.0$ & $4.5$ & $8.86\pm1.6$\\
J16370146$+$3535456 & $249.25609$ & $35.596016$ & $2881$ & $2800$ & $-0.0$ & $5.0$ & $<8.0$\\
J16383835$+$3700273 & $249.65982$ & $37.007591$ & $3288$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J16404891$+$3618596 & $250.20383$ & $36.316566$ & $3662$ & $3700$ & $+0.5$ & $5.0$ & $<8.0$\\
J16415893$+$3724468 & $250.49558$ & $37.413021$ & $3058$ & $3000$ & $+0.5$ & $5.5$ & $<8.0$\\
J16440030$+$3721597 & $251.00127$ & $37.366592$ & $3216$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J16454410$+$3605496 & $251.43379$ & $36.097115$ & $3312$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J16473499$+$3532388 & $251.89580$ & $35.544113$ & $3374$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J16495034$+$4745402 & $252.45977$ & $47.761181$ & $3719$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J16500047$+$4820372 & $252.50198$ & $48.343670$ & $3096$ & $3100$ & $-0.0$ & $5.5$ & $13.4\pm1.5$\\
J16541202$+$1154529 & $253.55011$ & $11.914707$ & $3788$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J16553439$+$0933530 & $253.89333$ & $9.5647230$ & $3891$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J16593773$+$1155377 & $254.90722$ & $11.927140$ & $3889$ & $4000$ & $-0.5$ & $4.5$ & $<8.0$\\
J17004418$+$1044240 & $255.18411$ & $10.740002$ & $3385$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J17014341$+$1119582 & $255.43090$ & $11.332844$ & $3539$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J17022763$+$1135227 & $255.61516$ & $11.589650$ & $3229$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J17033253$+$1015052 & $255.88558$ & $10.251469$ & $3822$ & $4000$ & $-0.5$ & $4.5$ & $<8.0$\\
J17150083$+$2246111 & $258.75346$ & $22.769751$ & $3545$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J17173369$+$2209028 & $259.39040$ & $22.150778$ & $3545$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J17190292$+$2340254 & $259.76217$ & $23.673731$ & $3778$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J17204248$+$4205070 & $260.17703$ & $42.085285$ & $3326$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J17212208$+$2326241 & $260.34200$ & $23.440042$ & $3819$ & $3900$ & $-0.5$ & $4.5$ & $<8.0$\\
J17295087$+$3501111 & $262.46198$ & $35.019772$ & $3705$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J17315986$+$7407420 & $262.99944$ & $74.128349$ & $3562$ & $3500$ & $+0.5$ & $5.0$ & $10.6\pm1.5$\\
J17331825$+$3402191 & $263.32607$ & $34.038647$ & $3897$ & $4000$ & $-0.5$ & $4.5$ & $<8.0$\\
J17335853$+$3610005 & $263.49390$ & $36.166824$ & $3624$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J17395925$+$3603304 & $264.99691$ & $36.058449$ & $3261$ & $3200$ & $+0.5$ & $5.0$ & $<8.0$\\
J17402294$+$3447423 & $265.09561$ & $34.795090$ & $3770$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J17403275$+$7256146 & $265.13647$ & $72.937393$ & $3887$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J17405641$+$3502205 & $265.23507$ & $35.039028$ & $3340$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J17413280$+$4808552 & $265.38669$ & $48.148674$ & $3410$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J17415545$+$3505012 & $265.48108$ & $35.083687$ & $3804$ & $3800$ & $-0.5$ & $4.5$ & $<8.0$\\
J17452435$+$6051259 & $266.35148$ & $60.857204$ & $3476$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J17460392$+$7351027 & $266.51636$ & $73.850761$ & $3392$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J17461184$+$6024225 & $266.54934$ & $60.406277$ & $3120$ & $3100$ & $-0.0$ & $5.0$ & $<8.0$\\
J17470130$+$4925053 & $266.75545$ & $49.418163$ & $3280$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J17471707$+$4715343 & $266.82113$ & $47.259537$ & $3755$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J17491402$+$4823093 & $267.30843$ & $48.385925$ & $3824$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J17491939$+$4649421 & $267.33079$ & $46.828388$ & $3322$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J17540504$+$6212016 & $268.52101$ & $62.200466$ & $3492$ & $3400$ & $-0.5$ & $4.5$ & $<8.0$\\
J17541820$+$4758412 & $268.57585$ & $47.978134$ & $3664$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J17545859$+$4715141 & $268.74416$ & $47.253929$ & $3394$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J17553826$+$6030011 & $268.90944$ & $60.500317$ & $3891$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J18071735$+$7402564 & $271.82231$ & $74.049004$ & $3943$ & $4000$ & $-0.0$ & $4.5$ & $<8.0$\\
J18161819$+$0131277 & $274.07582$ & $1.5243770$ & $3388$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J18163938$+$0047136 & $274.16411$ & $0.78713500$ & $3460$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J18164895$+$0150039 & $274.20398$ & $1.8344250$ & $3257$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J18215416$-$0700179 & $275.47567$ & $-7.0049820$ & $3881$ & $4000$ & $-0.0$ & $4.5$ & $<8.0$\\
J18231602$+$0058169 & $275.81676$ & $0.97138200$ & $3646$ & $3600$ & $-1.0$ & $4.5$ & $<8.0$\\
J18303947$-$0356189 & $277.66447$ & $-3.9385840$ & $3121$ & $3100$ & $-0.0$ & $5.0$ & $12.0\pm1.6$\\
J18405024$-$0804583 & $280.20934$ & $-8.0828830$ & $3274$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J18415473$+$0651285 & $280.47805$ & $6.8579410$ & $3458$ & $3400$ & $+0.5$ & $5.0$ & $<8.0$\\
J18523373$+$4538317 & $283.14055$ & $45.642147$ & $3094$ & $3200$ & $-0.5$ & $5.5$ & $<8.0$\\
J18551497$+$4408590 & $283.81241$ & $44.149742$ & $3264$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J18554773$+$0304254 & $283.94891$ & $3.0737270$ & $3659$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J18561502$+$0449049 & $284.06260$ & $4.8180390$ & $3613$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J18562628$+$4622532 & $284.10953$ & $46.381451$ & $3247$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J18571939$+$0523084 & $284.33082$ & $5.3856920$ & $3668$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J19003108$+$0422420 & $285.12953$ & $4.3783530$ & $3389$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J19004176$+$0310312 & $285.17403$ & $3.1753560$ & $3277$ & $3300$ & $-0.5$ & $4.5$ & $<8.0$\\
J19051739$+$4507161 & $286.32248$ & $45.121147$ & $3263$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J19071270$+$4416070 & $286.80293$ & $44.268635$ & $3210$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J19081576$+$2635054 & $287.06570$ & $26.584858$ & $3184$ & $3200$ & $-0.0$ & $5.5$ & $<8.0$\\
J19084251$+$2733453 & $287.17713$ & $27.562593$ & $3211$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J19094165$+$0948584 & $287.42356$ & $9.8162420$ & $3243$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J19103855$+$0132104 & $287.66063$ & $1.5362480$ & $3772$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J19121128$+$4316106 & $288.04701$ & $43.269630$ & $3380$ & $3400$ & $-0.5$ & $4.5$ & $<8.0$\\
J19125504$+$4239370 & $288.22936$ & $42.660290$ & $3585$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J19142151$+$4309008 & $288.58963$ & $43.150223$ & $2923$ & $3000$ & $-0.5$ & $5.5$ & $<8.0$\\
J19142401$+$1916006 & $288.60007$ & $19.266836$ & $3183$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J19142541$+$1755081 & $288.60591$ & $17.918922$ & $3877$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J19143925$+$1919025 & $288.66357$ & $19.317387$ & $3394$ & $3300$ & $+0.5$ & $4.5$ & $21.3\pm1.7$\\
J19170558$+$4007235 & $289.27329$ & $40.123199$ & $3388$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J19173151$+$2833147 & $289.38130$ & $28.554094$ & $3022$ & $3000$ & $-0.0$ & $5.5$ & $8.59\pm1.5$\\
J19182339$+$1839265 & $289.59748$ & $18.657368$ & $3382$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J19194106$+$4127490 & $289.92112$ & $41.463638$ & $2944$ & $3000$ & $-0.0$ & $5.5$ & $<8.0$\\
J19244226$+$4333498 & $291.17609$ & $43.563835$ & $3289$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J19264937$+$1643019 & $291.70573$ & $16.717199$ & $3384$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J19272650$+$4758468 & $291.86045$ & $47.979679$ & $3214$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J19281377$+$2459419 & $292.05738$ & $24.994986$ & $3856$ & $3900$ & $-0.0$ & $4.5$ & $<8.0$\\
J19294258$+$3733223 & $292.42745$ & $37.556198$ & $3145$ & $3200$ & $-0.0$ & $5.0$ & $9.09\pm1.6$\\
J19313868$-$0658253 & $292.91120$ & $-6.9737030$ & $3536$ & $3500$ & $+0.5$ & $5.0$ & $<8.0$\\
J19322564$+$3917266 & $293.10684$ & $39.290745$ & $2997$ & $3000$ & $-0.0$ & $5.0$ & $<8.0$\\
J19324633$-$0652178 & $293.19306$ & $-6.8716330$ & $3389$ & $3300$ & $+0.5$ & $4.5$ & $<8.0$\\
J19325604$+$1723567 & $293.23351$ & $17.399094$ & $3393$ & $3400$ & $-0.5$ & $4.5$ & $<8.0$\\
J19333940$+$3931372 & $293.41420$ & $39.527016$ & $3445$ & $3300$ & $-0.0$ & $4.5$ & $14.0\pm1.5$\\
J19335290$+$3900545 & $293.47045$ & $39.015152$ & $3195$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J19335405$+$3938497 & $293.47521$ & $39.647141$ & $3297$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J19341617$+$2553535 & $293.56741$ & $25.898218$ & $3342$ & $3400$ & $-0.5$ & $4.5$ & $<8.0$\\
J19380761$+$2316087 & $294.53174$ & $23.269106$ & $3169$ & $3300$ & $-1.5$ & $4.5$ & $<8.0$\\
J19390444$+$2424089 & $294.76851$ & $24.402493$ & $3475$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J19391233$+$1442505 & $294.80140$ & $14.714053$ & $3459$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J19412016$+$3912129 & $295.33401$ & $39.203602$ & $3422$ & $3500$ & $-0.0$ & $5.0$ & $<8.0$\\
J19412775$+$3239512 & $295.36564$ & $32.664223$ & $3379$ & $3400$ & $-0.5$ & $4.5$ & $<8.0$\\
J19430726$+$4518089 & $295.78028$ & $45.302483$ & $2948$ & $2800$ & $-0.0$ & $5.0$ & $<8.0$\\
J19433790$+$3225124 & $295.90793$ & $32.420135$ & $3984$ & $4000$ & $-0.0$ & $4.5$ & $19.7\pm1.5$\\
J19440865$+$2342587 & $296.03605$ & $23.716324$ & $3381$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J19454969$+$3223132 & $296.45707$ & $32.387005$ & $3623$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J19482428$+$3250327 & $297.10119$ & $32.842422$ & $3339$ & $3400$ & $-0.5$ & $4.5$ & $<8.0$\\
J19483064$+$2321473 & $297.12769$ & $23.363152$ & $3386$ & $3500$ & $-0.5$ & $5.0$ & $<8.0$\\
J19485718$+$5015245 & $297.23826$ & $50.256817$ & $3355$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J19491435$+$2421249 & $297.30982$ & $24.356932$ & $3308$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J19501592$+$3146598 & $297.56636$ & $31.783304$ & $3435$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J19504779$+$4816290 & $297.69915$ & $48.274731$ & $3301$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J19510930$+$4628598 & $297.78877$ & $46.483295$ & $3205$ & $3200$ & $-0.0$ & $5.0$ & $22.5\pm1.6$\\
J19535443$+$4424541 & $298.47680$ & $44.415043$ & $2749$ & $2600$ & $-0.0$ & $5.0$ & $22.6\pm1.5$\\
J19541829$+$1738289 & $298.57622$ & $17.641378$ & $3163$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J19551978$+$3029505 & $298.83245$ & $30.497370$ & $3500$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J19560585$+$2205242 & $299.02441$ & $22.090073$ & $3401$ & $3400$ & $+0.5$ & $5.5$ & $8.48\pm1.7$\\
J19591845$+$2040515 & $299.82689$ & $20.680998$ & $3288$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J20000520$+$0404424 & $300.02167$ & $4.0784470$ & $2880$ & $2800$ & $-0.5$ & $5.0$ & $<8.0$\\
J20014879$+$3122097 & $300.45332$ & $31.369387$ & $3090$ & $3000$ & $-0.0$ & $5.0$ & $13.5\pm1.6$\\
J20015056$+$4500500 & $300.46070$ & $45.013905$ & $3483$ & $3500$ & $+0.5$ & $5.5$ & $<8.0$\\
J20024041$+$3109447 & $300.66839$ & $31.162430$ & $3534$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J20032379$+$5549381 & $300.84917$ & $55.827271$ & $3101$ & $3100$ & $-0.0$ & $5.0$ & $<8.0$\\
J20032651$+$2952000 & $300.86050$ & $29.866682$ & $3146$ & $3100$ & $+0.5$ & $5.0$ & $<8.0$\\
J20053276$+$3039324 & $301.38650$ & $30.659004$ & $3790$ & $3900$ & $-0.5$ & $4.5$ & $<8.0$\\
J20082071$+$5444168 & $302.08631$ & $54.738010$ & $3333$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J20110664$+$2737093 & $302.77767$ & $27.619265$ & $3611$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J20122244$+$2043113 & $303.09352$ & $20.719828$ & $3431$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J20131291$+$2736152 & $303.30380$ & $27.604229$ & $3653$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J20141000$+$5546307 & $303.54169$ & $55.775200$ & $3269$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J20161339$+$1927287 & $304.05581$ & $19.457987$ & $3317$ & $3400$ & $-0.5$ & $4.5$ & $<8.0$\\
J20162519$+$5621561 & $304.10499$ & $56.365597$ & $3629$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J20185746$+$2704165 & $304.73943$ & $27.071264$ & $3585$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J20201596$+$2917103 & $305.06654$ & $29.286203$ & $3235$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J20262618$+$4419484 & $306.60911$ & $44.330112$ & $3272$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J20291663$+$4507525 & $307.31933$ & $45.131260$ & $3673$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J20295941$+$1709481 & $307.49758$ & $17.163382$ & $3403$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J20331096$+$4553299 & $308.29570$ & $45.891651$ & $3538$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J20351108$+$5426045 & $308.79618$ & $54.434608$ & $3416$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J20395260$+$4220335 & $309.96917$ & $42.342663$ & $3168$ & $3200$ & $-0.5$ & $4.5$ & $<8.0$\\
J20403814$+$4200055 & $310.15894$ & $42.001530$ & $3225$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J20405249$+$3219341 & $310.21873$ & $32.326149$ & $3664$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J20421377$+$3253473 & $310.55741$ & $32.896481$ & $3602$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J20425319$+$4243134 & $310.72163$ & $42.720409$ & $3236$ & $3300$ & $-0.5$ & $5.0$ & $<8.0$\\
J20440646$+$3409535 & $311.02696$ & $34.164879$ & $3125$ & $3100$ & $+0.5$ & $5.0$ & $<8.0$\\
J20452155$+$4216022 & $311.33981$ & $42.267281$ & $3080$ & $3100$ & $-0.0$ & $4.5$ & $43.6\pm1.5$\\
J20491376$+$3216514 & $312.30734$ & $32.280960$ & $2788$ & $3000$ & $-0.5$ & $5.5$ & $10.0\pm1.6$\\
J20491589$+$5203599 & $312.31624$ & $52.066639$ & $3575$ & $3600$ & $-0.5$ & $4.5$ & $<8.0$\\
J20492745$+$3336512 & $312.36440$ & $33.614227$ & $2765$ & $2800$ & $-0.0$ & $5.5$ & $<8.0$\\
J20504429$+$5059088 & $312.68457$ & $50.985786$ & $3317$ & $3400$ & $-0.5$ & $4.5$ & $<8.0$\\
J20511004$+$4254099 & $312.79184$ & $42.902752$ & $3254$ & $3300$ & $-0.5$ & $4.5$ & $<8.0$\\
J20563407$+$3929461 & $314.14197$ & $39.496140$ & $2956$ & $2900$ & $-0.5$ & $5.0$ & $<8.0$\\
J20584898$+$5115421 & $314.70409$ & $51.261696$ & $3543$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J21005978$+$5103147 & $315.24909$ & $51.054111$ & $3387$ & $3300$ & $-0.0$ & $4.5$ & $31.2\pm2.7$\\
J21013304$+$4046208 & $315.38769$ & $40.772449$ & $3258$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J21032130$+$2940340 & $315.83877$ & $29.676138$ & $3264$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J21074857$+$2945266 & $316.95241$ & $29.757389$ & $3517$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J21092552$+$4800013 & $317.35636$ & $48.000366$ & $3825$ & $4000$ & $-0.5$ & $4.5$ & $<8.0$\\
J21093969$+$4837150 & $317.41541$ & $48.620838$ & $2998$ & $2900$ & $-0.0$ & $5.5$ & $<8.0$\\
J21095447$+$4729043 & $317.47700$ & $47.484535$ & $3108$ & $3100$ & $-0.0$ & $5.0$ & $11.1\pm1.9$\\
J21095705$+$4811291 & $317.48774$ & $48.191425$ & $3325$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J21095952$+$4907498 & $317.49800$ & $49.130505$ & $3947$ & $4000$ & $-0.0$ & $4.5$ & $<8.0$\\
J21105881$+$4657325 & $317.74505$ & $46.959034$ & $3504$ & $3500$ & $+0.5$ & $5.0$ & $<8.0$\\
J21114023$+$2927586 & $317.91765$ & $29.466290$ & $3102$ & $3200$ & $-0.5$ & $5.5$ & $<8.0$\\
J21115993$+$4747251 & $317.99972$ & $47.790325$ & $3651$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J21160502$+$4759308 & $319.02095$ & $47.991913$ & $2712$ & $2900$ & $-0.0$ & $5.5$ & $15.0\pm1.7$\\
J21202943$+$4843460 & $320.12265$ & $48.729462$ & $3057$ & $3000$ & $+0.5$ & $5.0$ & $<8.0$\\
J21203355$+$4554475 & $320.13980$ & $45.913219$ & $3332$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J21215791$+$6742289 & $320.49133$ & $67.708038$ & $3164$ & $3100$ & $+0.5$ & $5.5$ & $<8.0$\\
J21223706$+$5555570 & $320.65443$ & $55.932514$ & $3415$ & $3500$ & $-0.5$ & $4.5$ & $10.4\pm1.5$\\
J21232573$+$6734153 & $320.85724$ & $67.570938$ & $3287$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J21274751$+$5505337 & $321.94797$ & $55.092705$ & $3219$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J21295287$+$4517484 & $322.47030$ & $45.296803$ & $3333$ & $3300$ & $+0.5$ & $5.0$ & $<8.0$\\
J21305987$+$5636274 & $322.74950$ & $56.607632$ & $3312$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J21321944$+$1052489 & $323.08104$ & $10.880258$ & $3406$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J21323014$+$4424296 & $323.12562$ & $44.408230$ & $3355$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J21325045$+$1206334 & $323.21023$ & $12.109280$ & $3577$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J21365219$+$4538240 & $324.21748$ & $45.640018$ & $3712$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J21375889$+$4201045 & $324.49540$ & $42.017921$ & $3714$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J21400112$+$5408179 & $325.00468$ & $54.138309$ & $3465$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J21400287$+$4123289 & $325.01198$ & $41.391369$ & $3534$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J21402935$+$5400301 & $325.12230$ & $54.008369$ & $3318$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J21442066$+$4211363 & $326.08612$ & $42.193432$ & $3281$ & $3300$ & $+0.5$ & $5.5$ & $12.9\pm1.6$\\
J21470874$+$5309448 & $326.78642$ & $53.162445$ & $3538$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J21474194$+$5341222 & $326.92478$ & $53.689518$ & $3699$ & $3700$ & $-0.0$ & $4.5$ & $<8.0$\\
J21481846$+$4131513 & $327.07694$ & $41.530941$ & $3802$ & $3700$ & $-0.5$ & $4.5$ & $<8.0$\\
J21551322$+$4938072 & $328.80511$ & $49.635349$ & $3426$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J21561443$+$3943468 & $329.06016$ & $39.729683$ & $3317$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J21563255$+$5335375 & $329.13565$ & $53.593765$ & $3402$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J21573509$+$5026323 & $329.39623$ & $50.442307$ & $3231$ & $3200$ & $+0.5$ & $5.5$ & $<8.0$\\
J21592435$+$4027339 & $329.85150$ & $40.459431$ & $3107$ & $3200$ & $-0.5$ & $5.5$ & $<8.0$\\
J21593422$+$5003575 & $329.89261$ & $50.065987$ & $3220$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J22010861$+$4901108 & $330.28589$ & $49.019684$ & $3951$ & $4000$ & $-0.0$ & $4.5$ & $<8.0$\\
J22011461$+$4008136 & $330.31088$ & $40.137135$ & $2628$ & $2600$ & $-0.0$ & $5.0$ & $9.46\pm1.6$\\
J22013085$+$6224408 & $330.37858$ & $62.411335$ & $3465$ & $3500$ & $-0.0$ & $5.0$ & $<8.0$\\
J22030336$+$6154513 & $330.76401$ & $61.914272$ & $3403$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J22111347$-$0232369 & $332.80613$ & $-2.5436040$ & $3591$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J22391615$+$0629545 & $339.81730$ & $6.4984910$ & $3412$ & $3300$ & $-0.0$ & $4.5$ & $<8.0$\\
J22431160$+$5228006 & $340.79834$ & $52.466850$ & $2986$ & $3000$ & $-0.0$ & $5.0$ & $9.32\pm1.6$\\
J22431234$+$0638221 & $340.80142$ & $6.6394760$ & $3793$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J22485465$+$0601251 & $342.22775$ & $6.0236550$ & $3607$ & $3600$ & $-0.0$ & $4.5$ & $<8.0$\\
J22502051$+$5136265 & $342.58548$ & $51.607388$ & $3075$ & $3000$ & $-0.0$ & $5.0$ & $11.1\pm1.5$\\
J22525818$+$5258468 & $343.24243$ & $52.979671$ & $3233$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J23034347$+$6524293 & $345.93114$ & $65.408165$ & $3265$ & $3300$ & $+0.5$ & $5.5$ & $<8.0$\\
J23053247$+$6543550 & $346.38531$ & $65.731964$ & $3422$ & $3500$ & $-0.5$ & $4.5$ & $<8.0$\\
J23062184$+$6503326 & $346.59104$ & $65.059074$ & $3199$ & $3200$ & $-0.5$ & $4.5$ & $<8.0$\\
J23062759$+$6352333 & $346.61499$ & $63.875927$ & $3332$ & $3300$ & $-0.0$ & $5.0$ & $<8.0$\\
J23081274$+$4609340 & $347.05309$ & $46.159466$ & $3230$ & $3200$ & $-0.0$ & $5.0$ & $<8.0$\\
J23082777$+$4700410 & $347.11573$ & $47.011395$ & $3227$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J23100304$+$6501022 & $347.51268$ & $65.017296$ & $3236$ & $3300$ & $-0.5$ & $5.0$ & $<8.0$\\
J23141283$+$6551158 & $348.55348$ & $65.854393$ & $3155$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J23165396$+$6109419 & $349.22487$ & $61.161652$ & $3614$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J23175293$+$6109518 & $349.47054$ & $61.164391$ & $3479$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J23185797$+$1042502 & $349.74156$ & $10.713948$ & $3410$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J23200542$+$6356068 & $350.02262$ & $63.935242$ & $3701$ & $3800$ & $-0.0$ & $4.5$ & $<8.0$\\
J23200936$+$1054252 & $350.03902$ & $10.907014$ & $3880$ & $4000$ & $-0.5$ & $4.5$ & $<8.0$\\
J23205304$+$1205009 & $350.22103$ & $12.083611$ & $3434$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J23213807$+$6442487 & $350.40863$ & $64.713547$ & $3191$ & $3200$ & $-0.0$ & $5.0$ & $8.72\pm1.7$\\
J23302492$+$6141107 & $352.60386$ & $61.686306$ & $3266$ & $3200$ & $-0.0$ & $4.5$ & $<8.0$\\
J23460112$+$7456172 & $356.50469$ & $74.938118$ & $3401$ & $3400$ & $-0.0$ & $5.0$ & $<8.0$\\
J23462781$+$7434098 & $356.61590$ & $74.569397$ & $3117$ & $3100$ & $-0.0$ & $4.5$ & $<8.0$\\
J23560029$+$1501409 & $359.00123$ & $15.028049$ & $3556$ & $3500$ & $+0.5$ & $5.0$ & $<8.0$\\
J23584065$+$7331547 & $359.66938$ & $73.531876$ & $3537$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
J23592059$+$1600146 & $359.83581$ & $16.004063$ & $3423$ & $3400$ & $-0.0$ & $4.5$ & $<8.0$\\
J23592772$+$1630288 & $359.86551$ & $16.508022$ & $3423$ & $3400$ & $+0.5$ & $5.5$ & $<8.0$\\
J23592810$+$7506017 & $359.86710$ & $75.100479$ & $3892$ & $4000$ & $-0.0$ & $4.5$ & $<8.0$\\
J23595589$+$1508091 & $359.98291$ & $15.135877$ & $3565$ & $3500$ & $-0.0$ & $4.5$ & $<8.0$\\
\enddata

